AET-SGD: Asynchronous Event-triggered Stochastic Gradient Descent

Communication cost is the main bottleneck for the design of effective distributed learning algorithms. Recently, event-triggered techniques have been proposed to reduce the exchanged information among compute nodes and thus alleviate the communication cost. However, most existing event-triggered approaches only consider heuristic event-triggered thresholds. They also ignore the impact of computation and network delay, which play an important role on the training performance. In this paper, we propose an Asynchronous Event-triggered Stochastic Gradient Descent (SGD) framework, called AET-SGD, to i) reduce the communication cost among the compute nodes, and ii) mitigate the impact of the delay. Compared with baseline event-triggered methods, AET-SGD employs a linear increasing sample size event-triggered threshold, and can significantly reduce the communication cost while keeping good convergence performance. We implement AET-SGD and evaluate its performance on multiple representative data sets, including MNIST, FashionMNIST, KMNIST and CIFAR10. The experimental results validate the correctness of the design and show a significant communication cost reduction from 44x to 120x, compared to the state of the art. Our results also show that AET-SGD can resist large delay from the straggler nodes while obtaining a decent performance and a desired speedup ratio.

==> Section/02_Dynamic_network_topology.tex <==
\section{Network topology: from static to dynamic}
\label{sec:topology}

\textbf{Problem formulation + Proposed Dynamic (controlled ) Network Topology}

% (1.5 pages)

==> Section/tikiz.tex <==
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}

\begin{document}

% \begin{tikzpicture}
% <code goes here>
% \end{tikzpicture}

\end{document}


